Verification of Deep Convolutional Neural Networks Using ImageStars

Convolutional Neural Networks (CNN) have redefined the state-of-the-art in many real-world applications, such as facial recognition, image classification, human pose estimation, and semantic segmentation. Despite their success, CNNs are vulnerable to adversarial attacks, where slight changes to their inputs may lead to sharp changes in their output in even well-trained networks. Set-based analysis methods can detect or prove the absence of bounded adversarial attacks, which can then be used to evaluate the effectiveness of neural network training methodology. Unfortunately, existing verification approaches have limited scalability in terms of the size of networks that can be analyzed. In this paper, we describe a set-based framework that successfully deals with real-world CNNs, such as VGG16 and VGG19, that have high accuracy on ImageNet. Our approach is based on a new set representation called the ImageStar, which enables efficient exact and over-approximative analysis of CNNs. ImageStars perform efficient set-based analysis by combining operations on concrete images with linear programming (LP). Our approach is implemented in a tool called NNV, and can verify the robustness of VGG networks with respect to a small set of input states, derived from adversarial attacks, such as the DeepFool attack. The experimental results show that our approach is less conservative and faster than existing zonotope methods, such as those used in DeepZ, and the polytope method used in DeepPoly.

==> ACASXu_tab.tex <==

% \usepackage{multirow}
\begin{table}[tbp]
   \centering
   \resizebox{0.7\linewidth}{!}{
\begin{tabular}{|l|l|c|l|l|l|l|l|l|c|}
\hline
\multirow{2}{*}{\textbf{Prop.}} & \multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Result}} & \multicolumn{5}{c|}{\textbf{NNV}} & \textbf{Reluplex} & \multirow{2}{*}{\textbf{r}} \\ \cline{4-9}
 &  &  & $N_s$ & $N_r$ & $RT(sec)$ & $ST(sec)$ & $VT(sec)$ & $VT (sec)$ &  \\ \hline
  \multirow{3}{*}{$\phi_1$} & $N_{1\_1}$ & SAFE & 39811 & 316528 & 1546.99 & 21.12  & 1568.11  & 5986 & 3.81x \\ \cline{2-10}
  & $N_{1\_2}$ &  SAFE & 45606 & 454369 & 1829.22 & 23.2  & 1852.42  & 6477 & 3.5x \\ \cline{2-10}
  & $N_{1\_3}$ &  SAFE & 114219 & 1220251 & 4786.63 & 64.71  & 4851.34  & 54800 & 11.3x \\ \hline
 \multirow{6}{*}{$\phi_3$} & $N_{1\_3}$ &  SAFE & 12274 & 56745 & 221.33 & 7.15  & 228.48  & 1102 & 4.82x \\ \cline{2-10}
  & $N_{2\_1}$ &  SAFE & 16179 & 98566 & 202.43 & 8.89  & 211.32  & 1173 & 5.55x \\ \cline{2-10}
  & $N_{2\_2}$ &  SAFE & 6861 & 3619 & 91.34 & 4.35  & 95.69  & 634 & 6.63x \\ \cline{2-10}
  & $N_{2\_3}$ &  SAFE & 10614 & 54784 & 152.94 & 5.9  & 158.84  & 1014 & 6.4x \\ \cline{2-10}
  & $N_{5\_1}$ &  SAFE & 9461 & 82353 & 138.72 & 5.84  & 144.56  & 1097 & 7.59x \\ \cline{2-10}
  & $N_{5\_3}$ &  SAFE & 2874 & 17078 & 57.04 & 2.38  & 59.42  & 338 & 5.7x \\ \hline

  \multirow{11}{*}{$\phi_4$} & $N_{1\_1}$ &  SAFE & 14066 & 22794 & 88.04 & 7.82  & 95.86  & 653 & 14.49x \\ \cline{2-10}
  & $N_{1\_2}$ &  SAFE & 6082 & 36246 & 76.12 & 3.98  & 80.1  & 1424 & 17.78x \\ \cline{2-10}
  & $N_{1\_3}$ &  SAFE & 4456 & 18656 & 71.34 & 3.23  & 74.57  & 1294 & 17.35x \\ \cline{2-10}
  & $N_{1\_5}$ &  SAFE & 760  & 10061 & 30.94 & 1.34  & 32.28  & 393 & 12.17x \\ \cline{2-10}
  & $N_{2\_2}$ &  SAFE & 2391 & 15251 & 32.87 & 2.24  & 35.11  & 451 & 12.84x \\ \cline{2-10}
  & $N_{2\_3}$ &  SAFE & 2357 & 11577 & 32.26 & 2.15  & 34.41  & 293 & 8.52x \\ \cline{2-10}
  & $N_{2\_8}$ &  SAFE & 421 & 6058 & 26.12 & 1.01  & 27.13  & 653 & 24.1x \\ \cline{2-10}
  & $N_{3\_7}$ &  SAFE & 203 & 3616 & 14.01 & 0.72  & 14.73  & 357 & 24.24x \\ \cline{2-10}
 & $N_{3\_9}$ &  SAFE & 657 & 12662 & 36.9 & 1.22  & 38.12  & 715 & 18.75x \\ \cline{2-10}
 & $N_{5\_1}$ &  SAFE & 931 & 6010 & 18.9 & 1.3  & 20.2  & 585 & 28.96x \\ \cline{2-10}
 & $N_{4\_9}$ &  SAFE & 286 & 7849 & 25.9 & 0.79  & 26.69  & 489 & 18.3x \\ \hline
$\phi_5$ & $N_{1\_1}$ &  SAFE & 193080 & 1755370 & 6555.49 & 97.6  & 6653.09 & 20448 & 3.1x \\ \hline
$\phi_7$ & $N_{1\_9}$ &  TIMEOUT &  &  &  &  &  & TIMEOUT &  \\ \hline
$\phi_{10}$ & $N_{4\_5}$ &  SAFE & 41088 & 226122 & 1906.17 & 21.26  & 1927.43 & 23917 & 12.41x \\ \hline
\multicolumn{9}{|l|}{Average Improvement in Verification Time:} & $\approx$ 12.2x \\ \hline
\end{tabular}}
\caption{Safety verification results on ACAS Xu networks in which $N_s$ is the number of stars in the reachable set, $N_r$ is the number of stepReLU operations reduced, $RT$ is the reachable set computation time, $ST$ is the safety checking time, $VT = RT + ST$ is the total verification time, and $r$ is the ratio of the verification times between NNV and Reluplex.}
\label{tab:ACASXu}
\vspace{-1em}
\end{table}

==> Implementation.tex <==
\section{Tool Architecture}
\vspace{-0.5em}
\seclabel{implementation}
\begin{figure}[t!]
\vspace{-1em}
  \centering
    \includegraphics[width=0.8\textwidth]{figures/NNV.pdf}
		\vspace{-1em}
   \caption{An overview of NNV.}
	\vspace{-1em}
   \label{fig:NNV}
 \end{figure}
%
NNV is an object-oriented toolbox which is built on top of the MPT toolbox \cite{kvasnica2004multi} and CORA \cite{althoff2015introduction} in Matlab. NNV makes use of the neural network model transformation tool (nnmt \footnote{https://github.com/verivital/nnmt}) which supports transforming neural network models from Keras and Tensorflow into Matlab using Open Neural Network Exachange format, and the hybrid systems model transformation and translation tool (HyST)~\cite{bak2015hyst} for plant configuration.
%
The NNV toolbox contains two main modules: a \emph{network engine} and an \emph{analyzer}, shown in Figure \ref{fig:NNV}.
The network engine module includes three subcomponents: 1) the \emph{feed-forward neural network (FFNN) constructor}, 2) the \emph{neural network control system (NNCS) constructor}, and 3) \emph{the star-based reachable set computation}. The FFNN constructor takes a network configuration file as an input and generates an FFNN object. The NNCS constructor takes the FFNN object and the Plant configuration which describes the dynamics of a system as inputs and then creates an NNCS object. Depends on application, either the FFNN object or the NNCS will be fed into the star-based reachable set computation to compute the reachable set of the neural network w.r.t a given initial condition. Then, the computed reachable will be inputted to the analyzer module. The analyzer module contains three subcomponents: 1) a \emph{visualizer}, 2) a \emph{safety checker}, and 3) a \emph{falsifier}. The visualizer can be called to plot the computed reachable set. Given a safety specification, the safety checker can reason about the safety of the FFNN w.r.t the specification. In the case of FFNN, the computed reachable set is the exact reachable set; thus the safety checker can return either safe or unsafe with a set of counterexamples. However, in the case of NNCS, the reachable set is an over-approximation of the actual reachable set. Therefore, the safety checker will return safe or uncertain. In the case of uncertain, NNV can call the falsifier to perform random simulations to falsify the safety property. The inputs of the falsifier are the safety specification and the NNCS object. If the falsifier can find a counterexample, then the NNCS is unsafe. Otherwise, it returns unknown.

%We note that NNV makes use the neural network model transformation tool (nnmt \footnote{https://github.com/verivital/nnmt}) which supports transforming neural network models from Keras and Tensorflow into Matlab using Open Neural Network Exachange format, and for closed-loop systems analysis, the hybrid systems model transformation and translation tool (HyST)~\cite{bak2015hyst}.

%the Layer, the ReLU and the Star classes. A feed-forward neural network is constructed using the constructor of FFNN class taking an array of Layer objects as input. The ReLU class contains methods for executing the stepReLU operation. A feedback NNCS is constructed using the constructor of the NNCS class taking FFNN and Plant objects as inputs. The Plant object describes the dynamics of the plant which can be linear or nonlinear ordinary differential equations (ODE). The Star class is a star set library implementing methods that are used in our reachability analysis algorithm such as affine mapping and half-space intersection. The cores of the FFNN and NNCS classes are the \emph{reach} methods which perform reachability analysis using star set. The computed reachable set is fed into the safety checker to reason about the safety of the FFNN or NNCS. In the case of NNCS, the reachable set is an over-approximation of the actual reachable set. Therefore, the safety checker returns safe or uncertain. In the case of uncertain, NNV can perform random simulations to falsify the safety property. If counterexamples are found, then the NNCS is unsafe. Otherwise, NNV returns unknown.


%NNV's core components are the feed-forward neural network (FFNN), the neural network control system (NNCS), the Layer, the ReLU and the Star classes. A feed-forward neural network is constructed using the constructor of FFNN class taking an array of Layer objects as input. The ReLU class contains methods for executing the stepReLU operation. A feedback NNCS is constructed using the constructor of the NNCS class taking FFNN and Plant objects as inputs. The Plant object describes the dynamics of the plant which can be linear or nonlinear ordinary differential equations (ODE). The Star class is a star set library implementing methods that are used in our reachability analysis algorithm such as affine mapping and half-space intersection. The cores of the FFNN and NNCS classes are the \emph{reach} methods which perform reachability analysis using star set. The computed reachable set is fed into the safety checker to reason about the safety of the FFNN or NNCS. In the case of NNCS, the reachable set is an over-approximation of the actual reachable set. Therefore, the safety checker returns safe or uncertain. In the case of uncertain, NNV can perform random simulations to falsify the safety property. If counterexamples are found, then the NNCS is unsafe. Otherwise, NNV returns unknown.

==> NNACC_tab.tex <==
\begin{table}[t!]
\vspace{-2em}
    \centering
   \resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{$\mathbf{x_{lead}(0)}$} & \multicolumn{2}{c|}{\textbf{Controller 1 (3x20)}} & \multicolumn{2}{c|}{\textbf{Controller 2 (5x20)}} & \multicolumn{2}{c|}{\textbf{Controller 3 (7x20)}} & \multicolumn{2}{c|}{\textbf{Controller 4(10x20)}} \\ \cline{2-9}
             & Result & VT (sec) & Result & VT (sec) & Result & VT (sec) & Result & VT (sec) \\ \hline
[108, 110]   & safe   & 211.84   & safe   & 292.67   & safe   & 398.41 & safe     & 1762  \\ \hline
{[}106, 108] & safe   & 210.16   & safe   & 288.83   & safe   & 393.35 & safe     & 2270.3 \\ \hline
[104, 106]   & safe   & 211.54   & safe   & 302.31   & safe   & 412.81 & safe     & 2674.5 \\ \hline
[102, 104]   & safe   & 215.21   & safe   & 292.94   & safe   & 446.47 & safe     & 2863.8 \\ \hline
[100, 102]   & safe   & 222.87   & safe   & 294.81   & safe   & 440.94 & safe     & 2606 \\ \hline
[98, 100]    & safe   & 233.02   & safe   & 302.74   & safe   & 491.29 & uncertain &2855  \\ \hline
[96, 98]     & safe   & 237.12   & safe   & 289.87   & safe   & 515.43 & uncertain &3249.9  \\ \hline
[94, 96]     & safe   & 238.46   & safe   & 301.99   & uncertain & 571.75  & uncertain & 3851.5  \\ \hline
[92, 94]     & safe   & 259.46   & safe   & 325.51   & uncertain & 598.22 & uncertain &  3220.2 \\ \hline
[90, 92]     & uncertain & 265.29& safe   & 359.92   & uncertain & 558.65 & uncertain &  2336.9 \\ \hline
\end{tabular}}
\vspace{1em}
\caption{Verification results for NNACC system with different neural network controllers in which $VT$ is the verification time and controller $k\times n$ means the controller has $k$ hidden layer and $n$ neuron per layer. The experiment is done on a desktop with following configuration: Intel Core i7-6700 CPU @ 3.4GHz $\times$ 8 Processor, 62.8 GiB Memory, 64-bit Ubuntu 16.04.3 LTS OS.}
\label{tab:NNACC}
\vspace{-1em}
\end{table}

==> NNACC_tab_falsification.tex <==
\begin{table}[t!]
    \centering
   \resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{$\mathbf{x_{lead}(0)}$} & \multicolumn{2}{c|}{\textbf{Controller 1 (3 x 20)}} & \multicolumn{2}{c|}{\textbf{Controller 2 (5 x 20)}} & \multicolumn{2}{c|}{\textbf{Controller 3 (7 x 20)}} & \multicolumn{2}{c|}{\textbf{Controller 4 (10 x 20)}} \\ \cline{2-9}
 & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} \\ \hline
[65, 70] & 100  & 43.63  & 303   & 45.25  & 486  & 46.91  & 134  & 49.13 \\ \hline
[70, 110] & 0  & 44.14  & 0     & 45.35  & 0    & 46.82  & 0    & 49.07 \\ \hline
\end{tabular}}
\caption{Falsification results for NNACC system with different neural network controllers using $1000$ random simulations in which $N_c$ is the number of counter examples and $FT$ is the falsification time.}
\label{tab:NNACC-falsification}
\vspace{-2em}
\end{table}

==> compare_tab.tex <==
\begin{table}[t!]
%\vspace{-2em}
    \centering
   \resizebox{\linewidth}{!}{
\setlength{\arrayrulewidth}{.15em}
\begin{tabular}{llll}
\hline
\textbf{Method} & \textbf{Input Size}      & \textbf{Data Set} & \textbf{Parameters} \\ \hline
MILP \cite{kouvaros2018formal}            & 28 x 28 x 1             & MNIST             & $1481$                          \\
DeepZono \cite{singh2018fast}        & 28 x 28 x1, 32 x 32 x 3 & MNIST, CIFAR10    & $88500$                         \\
DeepPoly \cite{singh2019abstract} & 28 x 28 x 1, 32 x 32 x3 & MNIST, CIFAR10    & $88500$                         \\
Simplex-based \cite{katz2019marabou}           & unevaluated             & unevaluated       & unevaluated                         \\
$L_0$ norm-based \cite{ruan2018global}           & \bf{224 x 224 x 3}    &  \bf{IMAGENET}    & $\mathbf{144000000}$    \\
\bf{ImageStar}           & \bf{224 x 224 x 3}               & \bf{IMAGENET}              & $\mathbf{144000000}$   \\
\hline
\end{tabular}}
%\vspace{1em}
\caption{Scalability of state-of-art approaches for convolutional neural network verification.}
\label{tab:compare}
\vspace{-1em}
\end{table}

==> ncs_verifiers.tex <==
\begin{table}[]
  \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Approaches} & \textbf{Plant Dynamics} & \textbf{Discrete/Continuous} & \textbf{Activation Function} & \textbf{Size of Controller} \\ \hline
Polyhedron-based \cite{xx} & Linear & Discrete & ReLU & $\leq$ 100 neurons \\ \hline
Verisig \cite{xx} & Linear, Nonlinear & Discrete, Continuous & Sigmoid, Tanh & $\leq$ 50 neurons \\ \hline
SMC-based \cite{xx} & Linear & Discrete & ReLU & $\leq$ 200 neurons \\ \hline
Sherlock \cite{xx} & Linear, Nonlinear & Discrete, Continuous & ReLU & $\leq$ 500 neurons \\ \hline
Star-based & Linear, Nonlinear & Discrete, Continuous & ReLU & $\leq$ 200 neurons \\ \hline
\end{tabular}}
\caption{Approaches for neural network control systems verification in which the sizes of controllers are collected from the related experimental results.}
\label{tab:ncs-verifiers}
\end{table}

==> preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
%
%\vspace{-0.25em}

\subsection{Problem definition}

A feed-forward neural network (FNN) consists of an input layer, an output layer, and multiple hidden layers in which each layer is comprised of neurons that are connected to the neurons of preceding layer labeled using weights \cite{hertz1991introduction}. Given an input vector, the output of an FNN is determined by three components: the weight matrices $W_{k,k-1}$, representing the weighted connection between neurons of two consecutive layers $k-1$ and $k$, the bias vectors $b_k$ of each layer, and the activation function $f$ applied at each layer. Mathematically, the output of a neuron $i$ is defined by:
%
\begin{equation*}
y_i = f(\Sigma_{j=1}^n\omega_{ij}x_j + b_i),
\end{equation*}
%
where $x_{j}$ is the $j^{th}$ input of the $i^{th}$ neuron, $\omega_{ij}$ is the weight from the $j^{th}$ input to the $i^{th}$ neuron, $b_i$ is the bias of the $i^{th}$ neuron. In this paper, we are interested in FNN with ReLU activation functions defined by $ReLU(x) = max(0, x)$.
%
%\begin{definition} [Layer Reachable Set] Given a bounded convex polyhedron input set defined as $I \triangleq \{x~|~Ax \leq b, x \in \mathbb{R}^n \}$, the reachable set of a layer $L$ with $m$ neurons corresponding to the input set $I$ is defined by:
  %
%  \begin{equation*}
%       R_{L} \triangleq \{y ~|~y = ReLU(Wx + b),~y \in \mathbb{R}^m, ~x \in I \},
%  \end{equation*}
%  where $W \in \mathbb{R}^{m \times n}$ and $b \in \mathbb{R}^m$ are the weights matrix and bias vector of the layer respectively.
%  %
%\end{definition}
%

\begin{definition}[Reachable Set of FNN]\label{def:reachable set} Given a bounded convex polyhedron input set defined as $\mathcal{I} \triangleq \{x~|~Ax \leq b, x \in \mathbb{R}^n \}$, and an $k$-layers feed-forward neural network $F \triangleq \{L_1, \cdots, L_k\}$, the reachable set $F(\mathcal{I}) = \mathcal{R}_{L_k}$ of the neural network $F$ corresponding to the input set I is defined incrementally by:
  \begin{equation*}
    \begin{split}
      \mathcal{R}_{L_{1}} &\triangleq \{y_1~|~y_1 = ReLU(W_1 x + b_1),~ x \in \mathcal{I}\}, \\
      \mathcal{R}_{L_{2}} &\triangleq \{y_2~|~y_2 = ReLU(W_2 y_1 + b_2),~ y_1 \in \mathcal{R}_{L_1}\}, \\
     &\vdots \\
    \mathcal{R}_{L_k} &\triangleq \{y_k ~|~ y_k = ReLU(W_k y_{k-1} + b_k)\,~y_{k-1} \in \mathcal{R}_{L_{k-1}} \}, \\
    \end{split}
  \end{equation*}
  where $W_k$ and $b_k$ are the weight matrix and bias vector of the $k^{th}$ layer $L_k$. The reachable set $\mathcal{R}_{L_k}$ contains all outputs of the neural network corresponding to all input vectors $x$ in the input set $\mathcal{I}$.

\end{definition}

\begin{definition}[Safety Verification of FNN] Given a $k$-layers feed-forward neural network $F$, and a safety specification $\mathcal{S}$ defined as a set of linear constraints on the neural network outputs $\mathcal{S} \triangleq \{y_k~|~Cy_k \leq d \}$, the neural network $F$ is called to be safe corresponding to the input set $\mathcal{I}$, we write $F(\mathcal{I}) \vDash S$, if and only if $\mathcal{R}_{L_k} \cap \neg \mathcal{S} = \emptyset$, where $\mathcal{R}_{L_k}$ is the reachable set of the neural network with the input set $\mathcal{I}$, and $\neg$ is the symbol for logical negation. Otherwise, the neural network is called to be unsafe $F(\mathcal{I}) \nvDash S$.
\end{definition}


\subsection{Generalized star sets}

\begin{definition}[Generalized Star Set \cite{bak2017simulation}] \label{def:star} A generalized star set (or simply star) $\Theta$ is a tuple $\langle c, V, P \rangle$ where $c \in \mathbb{R}^n$ is the center, $V = \{v_1, v_2, \cdots, v_m\}$ is a set of m vectors in $\mathbb{R}^n$ called basis vectors, and $P: \mathbb{R}^m \to \{ \top, \bot\}$ is a predicate. The basis vectors are arranged to form the star's $n \times m$ basis matrix. The set of states represented by the star is given as:
\begin{equation}
 \llbracket \Theta \rrbracket = \{x~|~x = c + \Sigma_{i=1}^m(\alpha_iv_i)~\text{such that}~P(\alpha_1, \cdots, \alpha_m) = \top \}.
\end{equation}
Sometimes we will refer to both the tuple $\Theta$ and the set of states $\llbracket \Theta \rrbracket$ as $\Theta$. In this work, we restrict the predicates to be a conjunction of linear constraints, $P(\alpha) \triangleq C\alpha \leq d$ where, for $p$ linear constraints, $C \in \mathbb{R}^{p \times m}$, $\alpha$ is the vector of $m$-variables, i.e., $\alpha = [\alpha_1, \cdots, \alpha_m]^T$, and $d \in \mathbb{R}^{p \times 1}$. A star is an empty set if and only if $P(\alpha)$ is empty.
\end{definition}

\begin{proposition} \label{pro1}
  Any bounded convex polyhedron $\mathcal{P} \triangleq \{x~|~Cx \leq d, x \in \mathbb{R}^n \}$ can be represented as a star.
\begin{proof}
    The polyhedron $\mathcal{P}$ is equivalent to the star set $\Theta$ with the center $c = [0, 0, \cdots, 0]^T$, the basic vectors $V = \{e_1, e_2, \cdots, e_n\}$ in which $e_i$ is the $i^{th}$ basic vector of $\mathbb{R}^n$, and the predicate $P(\alpha) \triangleq C\alpha \leq d$.
\end{proof}
\end{proposition}
%
\begin{proposition}[Affine Mapping of a Star]\label{pro2}
Given a star set $\Theta = \langle c, V, P\rangle$, an affine mapping of the star $\Theta$ with the affine mapping matrix $W$ and offset vector $b$ defined by $\bar{\Theta} = \{y~|~y=Wx + b,~x \in \Theta \}$ is another star with the following characteristics.
  \begin{equation*}
    \bar{\Theta} = \langle \bar{c}, \bar{V}, \bar{P} \rangle, ~ \bar{c} = Wc + b, ~\bar{v} = \{Wv_1, Wv_2, \cdots, Wv_m \},~ \bar{P} \equiv P.
  \end{equation*}
  \begin{proof}
    From the definition of a star, we have $\bar{\Theta} = \{y~|~y = Wc + b + \Sigma_{i=1}^m(\alpha_iWv_i),$ such that $~P(\alpha_1, \cdots, \alpha_m) = \top\}$ which implies that $\bar{\Theta}$ is another star with the center $\bar{c} = Wc + b$, basic vectors $\bar{V} =  \{Wv_1, Wv_2, \cdots, Wv_m \}$ and the same predicate $P$ as the original star $\Theta$.
  \end{proof}
\end{proposition}
%
\begin{proposition}[Star and Half-space Intersection]\label{pro:star intersection} The intersection of a star $\Theta \triangleq \langle c, V, P \rangle$ and a half-space $\mathcal{H} \triangleq \{x~|~Hx \leq g \}$ is another star with following characteristics.
  \begin{equation*}
    \begin{split}
      &\bar{\Theta} = \Theta \cap \mathcal{H} = \langle \bar{c}, \bar{V}, \bar{P} \rangle, ~\bar{c} = c,~\bar{V} = V, ~\bar{P} = P \wedge P^{\prime}, \\
      &P^{\prime}(\alpha) \triangleq (H\times V_m) \alpha \leq g - H \times c, V_m = [v_1~v_2 \cdots v_m].
    \end{split}
  \end{equation*}
  \begin{proof}
    For any $x \in \Theta \cap \mathcal{H}$, we have $x = c + \Sigma_{i=1}^m(\alpha_iv_i) \wedge Hx \leq g$, or equivalently, $x = c + \Sigma_{i=1}^m(\alpha_iv_i) \wedge H\times V_m \times \alpha \leq g - H\times c$ which implies that the intersection is another star with the same center $c$ and basic vectors $V$ as $\Theta$, and an updated predicate $\bar{P} = P \wedge P^{\prime}, P^{\prime}(\alpha) \triangleq  H\times V_m \times \alpha \leq g - H\times c$.
  \end{proof}
\end{proposition}

